Label, Verify, Correct: A Simple Few Shot Object Detection Method

The objective of this paper is few-shot object detection (FSOD) -- the task of expanding an object detector for a new category given only a few instances for training. We introduce a simple pseudo-labelling method to source high-quality pseudo-annotations from the training set, for each new category, vastly increasing the number of training instances and reducing class imbalance; our method finds previously unlabelled instances. Na\"ively training with model predictions yields sub-optimal performance; we present two novel methods to improve the precision of the pseudo-labelling process: first, we introduce a verification technique to remove candidate detections with incorrect class labels; second, we train a specialised model to correct poor quality bounding boxes. After these two novel steps, we obtain a large set of high-quality pseudo-annotations that allow our final detector to be trained end-to-end. Additionally, we demonstrate our method maintains base class performance, and the utility of simple augmentations in FSOD. While benchmarking on PASCAL VOC and MS-COCO, our method achieves state-of-the-art or second-best performance compared to existing approaches across all number of shots.

==> assets/tables/ablation.tex <==
% !TEX root = ../../main.tex
\begin{table*}[t]
\centering
\begin{adjustbox}{width=0.95\textwidth}
\begin{tabular}{@{}c|ccc|cccc|c|ccc|ccc@{}}
\toprule
\multirow{2}{*}{Model}  & \multicolumn{3}{c|}{Augmentation} & \multicolumn{4}{c|}{Finetune}                                                                                                                                                                                              & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ROI\\ Dropout\end{tabular}} & \multirow{2}{*}{nAP} & \multirow{2}{*}{nAP50} & \multirow{2}{*}{nAP75} & \multirow{2}{*}{nAPs} & \multirow{2}{*}{nAPm} & \multirow{2}{*}{nAPl} \\
                        &              \texttt{ColorJitter} & \texttt{RandomCrop} & \texttt{Mosaic}    & \begin{tabular}[c]{@{}c@{}}ROI\\ cls+reg\end{tabular} & \begin{tabular}[c]{@{}c@{}}ROI\\ fc1,fc2\end{tabular} & \begin{tabular}[c]{@{}c@{}}RPN\\ obj+reg\end{tabular} & \begin{tabular}[c]{@{}c@{}}RPN\\ conv\end{tabular} &                                                                             &                        &                       &                       &                       &                       &                      \\ \midrule
 A                      &                                   &                     &                    & \checkmark                                            &                                                       &                                                       &                                                    &                                                                             & 13.0                   & 24.7                  & 12.3                  & 5.5                   & 11.7                  & 19.8                 \\ \midrule
 B                      &              \checkmark           &                     &                    & \checkmark                                            &                                                       &                                                       &                                                    &                                                                             & 13.2                   & 24.9                  & 12.4                  & 5.6                   & 12.0                  & 20.2                 \\
 C                      &                                   & \checkmark          &                    & \checkmark                                            &                                                       &                                                       &                                                    &                                                                             & 13.2                   & 24.9                  & 12.6                  & 5.6                   & 11.7                  & 20.3                 \\
 D                      &                                   &                     & \checkmark         & \checkmark                                            &                                                       &                                                       &                                                    &                                                                             & 12.8                   & 24.1                  & 12.0                  & 6.1                   & 12.1                  & 18.9                 \\
 E                      &              \checkmark           & \checkmark          & \checkmark         & \checkmark                                            &                                                       &                                                       &                                                    &                                                                             & 13.8                   & 26.5                  & 13.2                  & 6.8                   & 14.1                  & 20.0                 \\ \midrule
 F                      &                                   &                     &                    & \checkmark                                            & \checkmark                                            &                                                       &                                                    &                                                                             & 13.0                   & 24.6                  & 12.3                  & 5.2                   & 11.8                  & 20.1                 \\
 G                      &                                   &                     &                    & \checkmark                                            &                                                       & \checkmark                                            &                                                    &                                                                             & 13.7                   & 26.4                  & 12.9                  & 5.6                   & 12.7                  & 20.6                 \\
 H                      &                                   &                     &                    & \checkmark                                            &                                                       & \checkmark                                            & \checkmark                                         &                                                                             & 14.2                   & 27.3                  & 13.3                  & 5.5                   & 13.4                  & 21.0                 \\
 I                      &                                   &                     &                    & \checkmark                                            & \checkmark                                            & \checkmark                                            & \checkmark                                         &                                                                             & 14.1                   & 27.5                  & 12.9                  & 4.0                   & 13.5                  & 22.7                 \\ \midrule
 J                      &              \checkmark           & \checkmark          & \checkmark         & \checkmark                                            &                                                       & \checkmark                                            & \checkmark                                         &                                                                             & 13.8                   & 26.5                  & 13.2                  & 6.8                   & 14.1                  & 20.0                 \\
 K                      &              \checkmark           & \checkmark          &                    & \checkmark                                            & \checkmark                                            & \checkmark                                            & \checkmark                                         &                                                                             & 14.5                   & 27.4                  & 13.9                  & 4.3                   & 13.0                  & 23.5                 \\
 L                      &              \checkmark           & \checkmark          & \checkmark         & \checkmark                                            & \checkmark                                            & \checkmark                                            & \checkmark                                         &                                                                             & 16.2                   & 30.0                  & 15.2                  & 6.4                   & 15.5                  & 24.6                 \\
 M                      &              \checkmark           & \checkmark          & \checkmark         & \checkmark                                            & \checkmark                                            & \checkmark                                            & \checkmark                                         & \checkmark                                                                  & \textbf{16.6}          & \textbf{30.9}         & \textbf{15.8}         &\textbf{ 7.0}          & \textbf{16.2}         & \textbf{24.8}        \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{
Ablation for various augmentations and finetuning strategies on the MS-COCO 30-shot task.}
\label{tab:ablation}
% \vspace{-20pt}
\end{table*}


==> assets/tables/ablation_backbone.tex <==
% !TEX root = ../../main.tex
\noindent
\begin{table}[htb!]
\centering
\scriptsize
% \vspace{-10pt}
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}l|c|ccc@{}}
\toprule
Model                             & Backbone                    & bAP  & bAP50 & bAP75 \\ \midrule
Base training only                & \multirow{3}{*}{ResNet-50}  & 37.7 & 57.9  & 41.3  \\
Baseline                          &                             & 29.5 & 46.7  & 32.4  \\
%Query Expansion             &                             & 24.0 & 37.1  & 26.8  \\
Query Expansion $\dagger$         &                             & 33.3 & 53.6  & 36.1  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-5pt}
\captionof{table}{Few-shot object detection performance on \textit{base} classes on the MS-COCO 30-shot task.
% Our baseline and query expansion models suffer from degradation in base class performance.
% Our query expansion$\dagger$ model recovers some base class performance.
}
\label{tab:ablation_base}
\end{table}
% \vspace{-10pt}


==> assets/tables/ablation_mid.tex <==
% !TEX root = ../../main.tex
\begin{table}[htb!]
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}c|ccc|c|c|c|c|@{}}
\toprule
\multirow{2}{*}{Setting} & \multicolumn{3}{c|}{Augmentations}                                                                                                                                     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Finetune\\ $\Phi_{\textsc{rpn}}$, $\Phi_{\textsc{roi}}$?\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\Phi_{\textsc{roi}}$\\ Dropout?\end{tabular}} & \multirow{2}{*}{nAP} & \multirow{2}{*}{nAPs} \\
                         & \begin{tabular}[c]{@{}c@{}}\texttt{Color}\\ \texttt{Jitter} \end{tabular} & \begin{tabular}[c]{@{}c@{}}\texttt{Random}\\ \texttt{Crop} \end{tabular} & \texttt{Mosaic} &                                                                                                                        &                                                                                           &                      &                       \\ \midrule
B1                       &                                                                           &                                                                          &                 &                                                                                                                        &                                                                                           & 13.0                 & 5.5                   \\
B2                       & \checkmark                                                                &                                                                          &                 &                                                                                                                        &                                                                                           & 13.2                 & 5.6                   \\
B3                       &                                                                           & \checkmark                                                               &                 &                                                                                                                        &                                                                                           & 13.2                 & 5.6                   \\
B4                       &                                                                           &                                                                          & \checkmark      &                                                                                                                        &                                                                                           & 12.8                 & 6.1                   \\
B5                       & \checkmark                                                                & \checkmark                                                               & \checkmark      &                                                                                                                        &                                                                                           & 13.8                 & 6.8                   \\ \midrule
C1                       & \checkmark                                                                & \checkmark                                                               &                 & \checkmark                                                                                                             &                                                                                           & 14.5                 & 4.3                   \\
C2                       & \checkmark                                                                & \checkmark                                                               & \checkmark      & \checkmark                                                                                                             &                                                                                           & 16.2                 & 6.2                   \\
C3                       & \checkmark                                                                & \checkmark                                                               & \checkmark      & \checkmark                                                                                                             & \checkmark                                                                                & 16.6                 & 7.0                   \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-5pt}
\captionof{table}{Few-shot object detection performance on \textit{base} classes on the MS-COCO 30-shot task.
Note that, the baseline model B1 is equivalent to a strong baseline proposed in TFA~\cite{Wang2020}.\vspace{-.5cm}}
\label{tab:ablation_mid}
\end{table}



==> assets/tables/ablation_mid_new.tex <==
% !TEX root = ../../main.tex
\begin{table*}[!htb]
\begin{minipage}[t]{0.46\linewidth}
\scriptsize
\setlength\tabcolsep{1.5pt}
\centering
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}[t]{@{}c|ccc|c|c|c|c|@{}}
\toprule
\multirow{2}{*}{Setting} & \multicolumn{3}{c|}{Augmentations}                                                                                                                                     & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Finetune\\ $\Phi_{\textsc{rpn}}$, $\Phi_{\textsc{roi}}$?\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\Phi_{\textsc{roi}}$\\ Dropout?\end{tabular}} & \multirow{2}{*}{nAP} & \multirow{2}{*}{nAPs} \\
\                        &  \begin{tabular}[c]{@{}c@{}}\texttt{Color}\\ \texttt{Jitter} \end{tabular} & \begin{tabular}[c]{@{}c@{}}\texttt{Random}\\ \texttt{Crop} \end{tabular} & \texttt{Mosaic} &                                                                                                                   &                                                                                           &                      &                       \\ \midrule
B1                       &                                                                           &                                                                          &                 &                                                                                                                   &                                                                                           & 13.0                 & 5.5                   \\
B2                       & \checkmark                                                                &                                                                          &                 &                                                                                                                   &                                                                                           & 13.2                 & 5.6                   \\
B3                       &                                                                           & \checkmark                                                               &                 &                                                                                                                   &                                                                                           & 13.2                 & 5.6                   \\
B4                       &                                                                           &                                                                          & \checkmark      &                                                                                                                   &                                                                                           & 12.8                 & 6.1                   \\
B5                       & \checkmark                                                                & \checkmark                                                               & \checkmark      &                                                                                                                   &                                                                                           & 13.8                 & 6.8                   \\ \midrule
C1                       & \checkmark                                                                & \checkmark                                                               &                 & \checkmark                                                                                                        &                                                                                           & 14.5                 & 4.3                   \\
C2                       & \checkmark                                                                & \checkmark                                                               & \checkmark      & \checkmark                                                                                                        &                                                                                           & 16.2                 & 6.2                   \\
C3                       & \checkmark                                                                & \checkmark                                                               & \checkmark      & \checkmark                                                                                                        & \checkmark                                                                                  & 16.6                 & 7.0                   \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-7pt}
\captionof{table}{Few-shot object detection performance on \textit{novel} classes on the MS-COCO 30-shot task.
Note that, the baseline model B1 is equivalent to a strong baseline proposed in TFA~\cite{Wang2020}.}
\label{tab:ablation_mid}

% \vspace{3pt}
\begin{adjustbox}{width=.98\columnwidth}
\begin{tabular}[t]{@{}l|ccc|ccc@{}}
\toprule
Method                           & nAP  & nAP50 & nAP75 & bAP  & bAP50 & bAP75 \\ \midrule
Baseline                         & 16.6 & 30.9  & 15.8  & 29.5 & 46.7  & 32.4  \\
+ Candidate Sourcing             & 18.4 & 34.0  & 18.2  & 31.7 & 53.2  & 35.6  \\
+ Label Verification             & 21.8 & 40.3  & 21.1  & 31.6 & 53.4  & 35.2  \\
+ Box Correction                 & 25.5 & 42.0  & 27.3  & 33.3 & 53.6  & 36.1  \\ \midrule
Ideal Faster R-CNN~\cite{Ren16}  & 43.5 & 67.4  & 46.6  & 36.1 & 56.0  & 39.2  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-7pt}
\captionof{table}{Ablation study on the proposed pseudo-labelling method.\vspace{-.2cm}}
\label{tab:ablation_qe_steps}
\end{minipage}
% ==================================================
\hfill
\begin{minipage}[t]{.52\linewidth}
\centering
\scriptsize
\begin{adjustbox}{width=\columnwidth}
\setlength\tabcolsep{2.5pt} % default value: 6pt
\begin{tabular}[t]{@{}l|c|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{Method}          & \multirow{2}{*}{Backbone}     & \multicolumn{2}{c|}{nAP}      & \multicolumn{2}{c|}{nAP50}      & \multicolumn{2}{c}{nAP75}      & \multicolumn{2}{c}{bAP}       \\
                                 &                               & 10            & 30            & 10             & 30             & 10             & 30            & 10           & 30             \\ \midrule
% FSRW~\cite{Kang2019}             & DarkNet-19                   & 5.6           & 9.1           & 12.3           & 19.0           & 4.6            & 7.6           & -            & -              \\ \midrule
CGDP+FSCN~\cite{Li2021}          &                               & 11.3          & 15.1          & 20.3           & 29.4           & -              & -             & -            & -              \\
\rowcolor[HTML]{EFEFEF}
Ours (Baseline)                  & ResNet-50                     & 11.4          & 16.6          & 21.2           & 30.9           & 11.1           & 15.8          & 28.4         & 29.5           \\
\rowcolor[HTML]{EFEFEF}
Ours (Pseudo-Labelling)          &                               & 17.6          & \best{25.5}   & \sbest{30.9}   & \best{42.0}    & \sbest{17.3}   & \best{27.3}   & 29.7         & 33.3           \\ \midrule
% MetaDet~\cite{Wang2019}          & \multirow{14}{*}{ResNet-101} & 7.1           & 11.3          & 14.6           & 21.7           & 6.1            & 8.1           & -            & -              \\
% Meta R-CNN~\cite{Yan2019}        &                              & 8.7           & 12.4          & 19.1           & 25.3           & 6.6            & 10.8          & -            & -              \\
% MPSR~\cite{Wu2020a}              &                              & 9.8           & 14.1          & 17.9           & 25.4           & 9.7            & 14.2          & -            & -              \\
% TFA w/ fc~\cite{Wang2020}        &                              & 10.0          & 13.4          & 19.2           & 24.7           & 9.2            & 13.2          & 32.0         & 33.8           \\
TFA w/ cos~\cite{Wang2020}       &                               & 10.0          & 13.7          & 19.1           & 24.9           & 9.3            & 13.4          & \sbest{32.4} & \sbest{34.2}   \\
FCSE~\cite{Sun2021}              &                               & 11.9          & 16.4          & -              & -              & 10.5           & 16.2          & -            & -              \\
Retentive R-CNN~\cite{Fan2021}   &                               & 10.5          & 13.8          & -              & -              & -              & -             & \best{39.2}  & \best{39.3}    \\
SRR-FSD~\cite{Zhu2021}           &                               & 11.3          & 14.7          & 23.0           & 29.2           & 9.8            & 13.5          & -            & -              \\
CME~\cite{Li2021b}               &                               & 15.1          & 16.9          & 24.6           & 28.0           & 16.4           & 17.8          & -            & -              \\
DCNet~\cite{Hu2021}              &                               & 12.8          & 18.6          & 23.4           & 32.6           & 11.2           & 17.5          & -            & -              \\
TIP~\cite{Li2021a}               &                               & 16.3          & 18.3          & \best{33.2}    & 35.9           & 14.1           & 16.9          & -            & -              \\
QA-FewDet~\cite{Han2021a}        &                               & 11.6          & 16.5          & 23.9           & 31.9           & 9.8            & 15.5          & -            & -              \\
FSOD-UP~\cite{Wu2021a}           &                               & 11.0          & 15.6          & -              & -              & 10.7           & 15.7          & -            & -              \\
DeFRCN$^*$~\cite{Qiao2021a}      &                               & \best{18.5}   & 22.6          & -              & -              & -              & -             & N/A          & N/A            \\
\rowcolor[HTML]{EFEFEF}
Ours (Baseline)                  &                               & 12.1          & 17.8          & 22.0           & 31.6           & 11.8           & 17.7          & 31.9         & 31.8           \\
\rowcolor[HTML]{EFEFEF}
Ours (Pseudo-Labelling)          & \multirow{-12}{*}{ResNet-101} & \sbest{17.8}  & \sbest{24.5}  & \sbest{30.9}   & \sbest{41.1}   & \best{17.8}    & \sbest{25.0}  & 31.9         & 33.0           \\ \midrule
\rowcolor[HTML]{C0C0C0}
Ours (Baseline)                  &                               & 12.6          & 19.0          & 23.3           & 35.3           & 12.1           & 18.3          & 27.2         & 31.5           \\
\rowcolor[HTML]{C0C0C0}
Ours (Pseudo-Labelling)          & \multirow{-2}{*}{Swin-T}      & 18.6          & 26.1          & 32.1           & 45.0           & 18.5           & 26.8          & 29.2         & 31.1           \\ \midrule
\rowcolor[HTML]{C0C0C0}
Ours (Baseline)                  &                               & 14.4          & 20.3          & 25.8           & 37.2           & 14.4           & 20.2          & 33.0         & 36.2           \\
\rowcolor[HTML]{C0C0C0}
Ours (Pseudo-Labelling)          & \multirow{-2}{*}{Swin-S}      & 19.0          & 26.8          & 34.1           & 45.8           & 19.0           & 27.5          & 28.7         & 34.8           \\ \bottomrule
% Ours (Query Expand 2x)  & \textit{}         & tbc           & 16.7          & tbc            & 31.1           & tbc            & 16.2          \\ \bottomrule
\end{tabular}
\end{adjustbox}
% \vspace{-2pt}
\captionof{table}{Few-shot detection performance on the MS-COCO benchmark.
We report performance on the 20 novel classes of MS-COCO in the FSOD setting.
Best and second-best results are coloured \best{blue} and \sbest{red}, respectively.
We additionally report performance on base classes. \vspace{-.2cm}}
% \vspace{-15pt}
\label{tab:coco_novel_post}
\end{minipage}
\end{table*}
% ==================================================




==> assets/tables/ablation_one-stage.tex <==
% !TEX root = ../../main.tex
\noindent
\begin{table}[h]
\centering
\scriptsize
% \vspace{-25pt}
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}l|c|ccc@{}}
\toprule
Model                    & Detector                       & nAP  & nAP50 & nAP75 \\ \midrule
Baseline                 & \multirow{2}{*}{Faster R-CNN}  & 16.6 & 30.9  & 15.8  \\
Query Expansion$\dagger$ &                                & 19.3 & 35.1  & 19.2  \\ \midrule
Baseline                 & \multirow{2}{*}{FCOS}          & 14.2 & 23.9  & 14.1  \\
Query Expansion$\dagger$ &                                & 17.8 & 28.9  & 18.2  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\captionof{table}{TO BE UPDATED IF INCLUDED Comparison between one-stage and two-stage detectors on the MS-COCO 30-shot task.}
\label{tab:ablation_one_stage}
\end{table}


==> assets/tables/ablation_simp.tex <==
% !TEX root = ../../main.tex
\begin{table}[htb!]
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}c|cc|c|ccc@{}}
\toprule
\multirow{2}{*}{Augment?} & \multicolumn{2}{c|}{Finetune?} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ROI\\ Dropout\end{tabular}} & \multirow{2}{*}{nAP} & \multirow{2}{*}{nAP50} & \multirow{2}{*}{nAP75} \\
                          & RPN            & ROI           &                                                                        &                      &                        &                        \\ \midrule
                          &                &               &                                                                        & 13.0                 & 24.7                   & 12.3                   \\ \midrule
\checkmark                &                &               &                                                                        & 13.8 (+0.8)          & 26.5 (+1.8)            & 13.2 (+0.9)            \\
                          & \checkmark     &               &                                                                        & 14.2 (+1.2)          & 27.3 (+2.6)            & 13.3 (+1.0)            \\
                          &                & \checkmark    &                                                                        & 13.3 (+0.3)          & 25.6 (+0.9)            & 12.6 (+0.3)            \\
                          & \checkmark     & \checkmark    &                                                                        & 14.3 (+1.3)          & 27.5 (+2.8)            & 12.9 (+0.6)            \\ \midrule
\checkmark                & \checkmark     & \checkmark    &                                                                        & 16.2 (+3.3)          & 30.0 (+5.3)            & 15.2 (+2.9)            \\
\checkmark                & \checkmark     & \checkmark    & \checkmark                                                             & 16.6 (+3.6)          & 30.9 (+6.2)            & 15.8 (+3.5)            \\ \bottomrule
\end{tabular}
\end{adjustbox}
\captionof{table}{Few-shot object detection performance on \textit{base} classes on the MS-COCO 30-shot task.
% Our baseline and query expansion models suffer from degradation in base class performance.
% Our query expansion$\dagger$ model recovers some base class performance.
}
\label{tab:ablation_simp}
\end{table}



==> assets/tables/coco_full.tex <==
% !TEX root = ../../main.tex
\begin{table*}[]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}c|c|c|cccccc|ccc|ccc@{}}
\toprule
\multirow{2}{*}{\# shots} & \multirow{2}{*}{Method}      & \multirow{2}{*}{Backbone} & \multicolumn{6}{c|}{Overall}            & \multicolumn{3}{c|}{Base class} & \multicolumn{3}{c}{Novel class} \\
                          &                              &                                & AP   & AP50 & AP75 & APs  & APm  & APl  & AP        & AP50     & AP75     & AP        & AP50     & AP75     \\ \midrule
\multirow{9}{*}{10}       & FR~\cite{Kang2019}           & YOLOv2 w/ DarkNet-19           & -    & -    & -    & -    & -    & -    & -         & -        & -        & 5.6       & 12.3     & 4.6      \\
                          & MetaDet~\cite{Wang2019}      & FRCN w/ VGG16                  & -    & -    & -    & -    & -    & -    & -         & -        & -        & 7.1       & 14.6     & 6.1      \\ \cmidrule(lr){2-15}
                          & Meta R-CNN~\cite{Yan2019}    & \multirow{5}{*}{FPN w/ R-101}  & -    & -    & -    & -    & -    & -    & -         & -        & -        & 8.7       & 19.1     & 6.6      \\
                          & FRCN-ft-full~\cite{Wang2020} &                                & 13.4 & 21.8 & 14.5 & 5.1  & 14.3 & 20.1 & 16.1      & 25.7     & 17.5     & 5.5       & 10.0     & 5.5      \\
                          & TFA w/ fc~\cite{Wang2020}    &                                & 26.2 & 41.8 & 28.6 & 14.5 & 29.0 & 35.2 & 32.0      & 49.9     & 35.3     & 9.1       & 17.3     & 8.5      \\
                          & TFA w/ cos~\cite{Wang2020}   &                                & 26.6 & 42.2 & 29.0 & 15.0 & 29.1 & 35.2 & 32.4      & 50.6     & 35.7     & 9.1       & 17.1     & 8.8      \\
                          & FSOD-VE~\cite{Xiao2020}      &                                & -    & -    & -    & -    & -    & -    & -         & -        & -        & 12.5      & 27.3     & 9.8      \\ \cmidrule(lr){2-15}
                          & Ours (stage-1 training)      & \multirow{2}{*}{FPN w/ R-50}   & -    & -    & -    & -    & -    & -    & 30.4      & 48.0     & 32.0     & -         & -        & -        \\
                          & Ours (finetune)              &                                & 22.7 & 36.7 & 23.7 & 12.0 & 25.8 & 31.9 & 28.6      & 45.8     & 30.1     & 4.9       & 10.4     & 4.3      \\ \midrule
\multirow{9}{*}{30}       & FR~\cite{Kang2019}           & YOLOv2 w/ DarkNet-19           & -    & -    & -    & -    & -    & -    & -         & -        & -        & 9.1       & 19.0     & 7.6      \\
                          & MetaDet~\cite{Wang2019}      & FRCN w/ VGG16                  & -    & -    & -    & -    & -    & -    & -         & -        & -        & 11.3      & 21.7     & 8.1      \\ \cmidrule(lr){2-15}
                          & Meta R-CNN~\cite{Yan2019}    & \multirow{5}{*}{FRCN w/ R-101} & -    & -    & -    & -    & -    & -    & -         & -        & -        & 12.4      & 25.3     & 10.8     \\
                          & FRCN-ft-full~\cite{Wang2020} &                                & 13.5 & 21.8 & 14.5 & 5.1  & 14.6 & 19.9 & 15.6      & 24.8     & 16.9     & 7.4       & 13.1     & 7.4      \\
                          & TFA w/ fc~\cite{Wang2020}    &                                & 28.4 & 44.4 & 31.2 & 15.7 & 31.2 & 38.6 & 33.8      & 51.8     & 37.6     & 12.0      & 22.2     & 11.8     \\
                          & TFA w/ cos~\cite{Wang2020}   &                                & 28.7 & 44.7 & 31.5 & 16.1 & 31.2 & 38.4 & 34.2      & 52.3     & 38.0     & 12.1      & 22.0     & 12.0     \\
                          & FSOD-VE~\cite{Xiao2020}      &                                & -    & -    & -    & -    & -    & -    & -         & -        & -        & 14.7      & 30.6     & 12.2     \\ \cmidrule(lr){2-15}
                          & Ours (stage-1 training)      & \multirow{2}{*}{FPN w/ R-50}   & -    & -    & -    & -    & -    & -    & 30.4      & 48.0     & 32.0     & -         & -        & -        \\
                          & Ours (finetune)              &                                & 24.0 & 39.0 & 24.9 & 13.1 & 26.9 & 33.3 & 29.2      & 46.6     & 30.7     & 8.2       & 16.1     & 7.3      \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{3pt}
\caption{TO BE UPDATED Detailed few-shot object detection performance on the MS-COCO dataset.
         Our initial results demonstrate promising performance on novel classes.
         Moreover, we show that base class performance does not reduce appreciably when finetuning on novel classes.}
\label{tab:coco_full}
\end{table*}
% 12.5588,26.3124,31.3252


==> assets/tables/coco_novel.tex <==
% !TEX root = ../../main.tex
\begin{table}[t]
\centering
\begin{tabular}{@{}cl|ccc@{}}
\toprule
\multirow{2}{*}{Shots} & \multirow{2}{*}{Method}    & \multicolumn{3}{c}{Novel AP} \\
                       &                            & 0.5:0.95        & 0.5           & 0.75            \\ \midrule
                       & FR~\cite{Kang2019}         & 5.6             & 12.3          & 4.6             \\
                       & MetaDet~\cite{Wang2019}    & 7.1             & 14.6          & 6.1             \\
                       & Meta R-CNN~\cite{Yan2019}  & 8.7             & 19.1          & 6.6             \\
10                     & TFA w/ fc~\cite{Wang2020}  & 9.1             & 17.3          & 8.5             \\
                       & TFA w/ cos~\cite{Wang2020} & 9.1             & 17.1          & 8.8             \\
                       & FSOD-VE~\cite{Xiao2020}    & \textbf{12.5}   & \textbf{27.3} & \textbf{9.8}    \\
                       & Ours                       & 4.9             & 10.4          & 4.3             \\ \midrule
                       & FR~\cite{Kang2019}         & 9.1             & 19.0          & 7.6             \\
                       & MetaDet~\cite{Wang2019}    & 11.3            & 21.7          & 8.1             \\
                       & Meta R-CNN~\cite{Yan2019}  & 12.4            & 25.3          & 10.8            \\
30                     & TFA w/ fc~\cite{Wang2020}  & 12.0            & 22.2          & 11.8            \\
                       & TFA w/ cos~\cite{Wang2020} & 12.1            & 22.0          & 12.0            \\
                       & FSOD-VE~\cite{Xiao2020}    & \textbf{14.7}   & \textbf{30.6} & \textbf{12.2}   \\
                       & Ours                       & -               & -      & -      \\ \bottomrule
\end{tabular}
\vspace{3pt}
\caption{Few-shot detection performance the MS-COCO dataset. We report performance on the 20 novel classes of COCO in the few-shot object detection setting.}
\label{tab:coco_novel}
\end{table}


==> assets/tables/coco_novel_bmvc.tex <==
% !TEX root = ../../main.tex
\begin{minipage}[htb!]{0.6\textwidth}
\centering
\scriptsize
\vspace{25pt}
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}l|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{Method}        & \multicolumn{2}{c|}{nAP} & \multicolumn{2}{c|}{nAP50} & \multicolumn{2}{c}{nAP75} \\
                                & 10            & 30            & 10             & 30             & 10             & 30            \\ \midrule
FSRW~\cite{Kang2019}        \hfill \textit{ICCV 19}  & 5.6           & 9.1           & 12.3           & 19.0           & 4.6            & 7.6           \\
MetaDet~\cite{Wang2019}     \hfill \textit{ICCV 19}  & 7.1           & 11.3          & 14.6           & 21.7           & 6.1            & 8.1           \\
Meta-RCNN~\cite{Yan2019}    \hfill \textit{ICCV 19}  & 8.7           & 12.4          & 19.1           & 25.3           & 6.6            & 10.8          \\
MPSR~\cite{Wu2020a}         \hfill \textit{ECCV 20}  & 9.8           & 14.1          & 17.9           & 25.4           & 9.7            & 14.2          \\
TFA w/ fc~\cite{Wang2020}   \hfill \textit{ICML 20}  & 10.0          & 13.4          & 19.2           & 24.7           & 9.2            & 13.2          \\
TFA w/ cos~\cite{Wang2020}  \hfill \textit{ICML 20}  & 10.0          & 13.7          & 19.1           & 24.9           & 9.3            & 13.4          \\
FCSE~\cite{Sun2021}         \hfill \textit{CVPR 21}  & \sbest{11.9}  & 16.4          & -              & -              & 10.5           & \sbest{16.2}  \\
Retentive R-CNN~\cite{Fan2021} \hfill \textit{CVPR 21}  & 10.5          & 13.8          & -              & -              & -              & -             \\ \midrule
Ours (Baseline)             \hfill \textit{}         & 11.6          & \sbest{16.6}  & \best{22.3}    & \best{30.9}    & \sbest{11.0}   & 15.8          \\
Ours (After Query Expansion)           \textit{}         & \best{12.4}   & \best{17.5}   & \sbest{22.1}   & \sbest{30.2}   & \best{12.6}    & \best{17.8}   \\ \bottomrule
% Ours (Query Expand 2x)  & \textit{}         & tbc           & 16.7          & tbc            & 31.1           & tbc            & 16.2          \\ \bottomrule
\end{tabular}
\end{adjustbox}
% \vspace{3pt}
\captionof{table}{Few-shot detection performance on the MS-COCO benchmark.
We report performance on the 20 novel classes of MS-COCO in the FSOD setting.
Best and second-best results are coloured \best{blue} and \sbest{red},
respectively}
% \vspace{-15pt}
\label{tab:coco_novel}
\end{minipage}
\hfill
\begin{minipage}[htb!]{0.38\textwidth}
\centering
\vspace{12pt}
\includegraphics[width=\linewidth]{assets/images/NewDets.png}
\captionof{figure}{New detections \textit{after query expansion} for PASCAL VOC Split 2 with $K=1$.}
\label{fig:qe_new_dets}
\end{minipage}


==> assets/tables/coco_novel_bmvc_post.tex <==
% !TEX root = ../../main.tex
\noindent
\begin{table}[t]
\centering
\scriptsize
%\vspace{25pt}
\begin{adjustbox}{width=\columnwidth}
\setlength\tabcolsep{3.5pt} % default value: 6pt
\begin{tabular}{@{}l|c|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{Method}          & \multirow{2}{*}{Backbone}    & \multicolumn{2}{c|}{nAP}      & \multicolumn{2}{c|}{nAP50}      & \multicolumn{2}{c}{nAP75}      & \multicolumn{2}{c}{bAP}       \\
                                 &                              & 10            & 30            & 10             & 30             & 10             & 30            & 10           & 30             \\ \midrule
FSRW~\cite{Kang2019}             & DarkNet-19                   & 5.6           & 9.1           & 12.3           & 19.0           & 4.6            & 7.6           & -            & -              \\ \midrule
CGDP+FSCN~\cite{Li2021}          &                              & 11.3          & 15.1          & 20.3           & 29.4           & -              & -             & -            & -              \\
\rowcolor[HTML]{EFEFEF}
Ours (Baseline)                  & ResNet-50                    & 11.4          & 16.6          & 21.2           & 30.9           & 11.1           & 15.8          & 28.4         & 29.5           \\
\rowcolor[HTML]{EFEFEF}
Ours (Pseudo-Labelling)          &                              & 17.6          & \best{25.5}   & \sbest{30.9}   & \best{42.0}    & \sbest{17.3}   & \best{27.3}   & 29.7         & 33.3           \\ \midrule
MetaDet~\cite{Wang2019}          & \multirow{14}{*}{ResNet-101} & 7.1           & 11.3          & 14.6           & 21.7           & 6.1            & 8.1           & -            & -              \\
Meta R-CNN~\cite{Yan2019}        &                              & 8.7           & 12.4          & 19.1           & 25.3           & 6.6            & 10.8          & -            & -              \\
MPSR~\cite{Wu2020a}              &                              & 9.8           & 14.1          & 17.9           & 25.4           & 9.7            & 14.2          & -            & -              \\
TFA w/ fc~\cite{Wang2020}        &                              & 10.0          & 13.4          & 19.2           & 24.7           & 9.2            & 13.2          & 32.0         & 33.8           \\
TFA w/ cos~\cite{Wang2020}       &                              & 10.0          & 13.7          & 19.1           & 24.9           & 9.3            & 13.4          & \sbest{32.4} & \sbest{34.2}   \\
FCSE~\cite{Sun2021}              &                              & 11.9          & 16.4          & -              & -              & 10.5           & 16.2          & -            & -              \\
Retentive R-CNN~\cite{Fan2021}   &                              & 10.5          & 13.8          & -              & -              & -              & -             & \best{39.2}  & \best{39.3}    \\
SRR-FSD~\cite{Zhu2021}           &                              & 11.3          & 14.7          & 23.0           & 29.2           & 9.8            & 13.5          & -            & -              \\
CME~\cite{Li2021b}               &                              & 15.1          & 16.9          & 24.6           & 28.0           & 16.4           & 17.8          & -            & -              \\
DCNet~\cite{Hu2021}              &                              & 12.8          & 18.6          & 23.4           & 32.6           & 11.2           & 17.5          & -            & -              \\
TIP~\cite{Li2021a}               &                              & 16.3          & 18.3          & \best{33.2}    & 35.9           & 14.1           & 16.9          & -            & -              \\
QA-FewDet~\cite{Han2021a}        &                              & 11.6          & 16.5          & 23.9           & 31.9           & 9.8            & 15.5          & -            & -              \\
FSOD-UP~\cite{Wu2021a}           &                              & 11.0          & 15.6          & -              & -              & 10.7           & 15.7          & -            & -              \\
DeFRCN$^*$~\cite{Qiao2021a}      &                              & \best{18.5}   & 22.6          & -              & -              & -              & -             & N/A          & N/A            \\
\rowcolor[HTML]{EFEFEF}
Ours (Baseline)                  &                              & 12.1          & 17.8          & 22.0           & 31.6           & 11.8           & 17.7          & 31.9         & 31.8           \\
\rowcolor[HTML]{EFEFEF}
Ours (Pseudo-Labelling)          &                              & \sbest{17.8}  & \sbest{24.5}  & \sbest{30.9}   & \sbest{41.1}   & \best{17.8}    & \sbest{25.0}  & 31.9         & 33.0           \\ \midrule
\rowcolor[HTML]{EFEFEF}
Ours (Baseline)                  &                              & 12.6          & 19.0          & 23.3           & 35.3           & 12.1           & 18.3          & 27.2         & 31.5           \\
\rowcolor[HTML]{EFEFEF}
Ours (Pseudo-Labelling)          & \multirow{-2}{*}{Swin-T}     & 18.6          & 26.1          & 32.1           & 45.0           & 18.5           & 26.8          & 29.2         & 31.1           \\ \midrule
\rowcolor[HTML]{EFEFEF}
Ours (Baseline)                  &                              & 14.4          & 20.3          & 25.8           & 37.2           & 14.4           & 20.2          & 33.0         & 36.2           \\
\rowcolor[HTML]{EFEFEF}
Ours (Pseudo-Labelling)          & \multirow{-2}{*}{Swin-S}     & 19.0          & 26.8          & 34.1           & 45.8           & 19.0           & 27.5          & 28.7         & 34.8           \\ \bottomrule
% Ours (Query Expand 2x)  & \textit{}         & tbc           & 16.7          & tbc            & 31.1           & tbc            & 16.2          \\ \bottomrule
\end{tabular}
\end{adjustbox}
% \vspace{3pt}
\captionof{table}{Few-shot detection performance on the MS-COCO benchmark.
We report performance on the 20 novel classes of MS-COCO in the FSOD setting.
Best and second-best results are coloured \best{blue} and \sbest{red},
respectively}
% \vspace{-15pt}
\label{tab:coco_novel_post}
\end{table}


\begin{figure*}[!htb]
\centering
\scriptsize
% \begin{minipage}[b]{0.48\linewidth}
\includegraphics[width=\linewidth]{assets/images/verify_correct.eps}
\caption{\hl{TO DO}}
% \vspace{-0.65cm}
\label{fig:verify_correct}
% \vspace{-0.7cm}
\end{figure*}

%\begin{figure}[h]
%\centering
% \vspace{-18pt}
%\includegraphics[width=\linewidth]{assets/images/NewDets.png}
%\captionof{figure}{New detections \textit{after query expansion} for PASCAL VOC Split 2 with $K=1$. \hl{to be removed or changed}}
%\label{fig:qe_new_dets_post}
%\end{figure}

% \vspace{3pt}


==> assets/tables/lvis_full.tex <==
% !TEX root = ../../main.tex
\begin{table*}[ht]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}c|c|c|ccc|ccc|ccc@{}}
\toprule
Method         & Backbone                      & Repeated sampling                          & AP   & AP50 & AP75 & APs  & APm  & APl  & APr  & APc  & APf  \\ \midrule
Joint training~\cite{Gupta2019} & \multirow{3}{*}{FRCN w/ R-50} & \multirow{3}{*}{}                          & 19.8 & 33.6 & 20.4 & 17.1 & 25.9 & 33.2 & 2.1  & 18.5 & 28.5 \\
TFA w/ fc~\cite{Wang2020}       &                               &                                            & 22.3 & 37.8 & 22.2 & 18.5 & 28.2 & 36.6 & 14.3 & 21.1 & 27.0 \\
TFA w/ cos~\cite{Wang2020}      &                               &                                            & 22.7 & 37.2 & 23.9 & 18.8 & 27.7 & 37.1 & 15.4 & 2.5  & 28.4 \\ \midrule
Ours                            & FCOS w/ R-50                  &                                            & -    & -    & -    & -    & -    & -    & -    & -    & -    \\ \midrule
Joint training~\cite{Gupta2019} & \multirow{3}{*}{FRCN w/ R-50} & \multirow{3}{*}{\checkmark}                & 23.1 & 38.4 & 24.3 & 18.1 & 28.3 & 36.0 & 13.0 & 22.0 & 28.4 \\
TFA w/ fc~\cite{Wang2020}       &                               &                                            & 24.1 & 39.9 & 25.4 & 19.5 & 29.1 & 36.7 & 14.9 & 23.9 & 27.9 \\
TFA w/ cos~\cite{Wang2020}      &                               &                                            & 24.4 & 40.0 & 26.1 & 19.9 & 29.5 & 38.2 & 16.9 & 24.3 & 27.7 \\ \midrule
Ours                            & FPN w/ R-50                  & \checkmark                                 & -    & -    & -    & -    & -    & -    & -    & -    & -    \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{3pt}
\caption{Few-shot object detection performance on the LVIS dataset.
         We compare our approach to the dataset baseline provided by~\cite{Gupta2019} and to the approach in~\cite{Wang2020}.
         Furthermore, we illustrate the necessity of repeated sampling (a technique used in~\cite{Gupta2019}) on joint training, in contrast to our approach.
         Presented baselines use the two-stage Faster R-CNN detector, whereas we use a model inspired by FCOS.
         All models use a ResNet-50 backbone for fair comparisons.}
\label{tab:lvis_full}
\end{table*}


==> assets/tables/pascal_base.tex <==
% !TEX root = ../../main.tex
\begin{table}[]
\centering
\begin{tabular}{@{}c|c|cc@{}}
\toprule
\# shots            & Method           & Base AP50 & Novel AP50 \\ \midrule
\multirow{5}{*}{3}  & Meta R-CNN~\cite{Yan2019}    & 64.8      & 35.0       \\
                    & FRCN-ft-full~\cite{Wang2020} & 66.1      & 29.0       \\
                    & TFA w/ cos~\cite{Wang2020}   & 79.1      & 44.7       \\
                    & Ours (base only)             & -         & -          \\
                    & Ours                         & -         & -          \\ \midrule
\multirow{5}{*}{10} & Meta R-CNN~\cite{Yan2019}    & 67.9      & 51.5       \\
                    & FRCN-ft-full~\cite{Wang2020} & 66.0      & 45.5       \\
                    & TFA w/ cos~\cite{Wang2020}   & 78.4      & 56.0       \\
                    & Ours (base only)             & -         & -          \\
                    & Ours                         & -         & -          \\ \bottomrule
\end{tabular}
\vspace{3pt}
\caption{Few-shot object detection performance on novel set 1 on the Pascal VOC dataset.
         Our model outperforms previous approaches on both base and novel classes.
         Furthermore, we demonstrate that finetuning on novel classes does not degrade base class performance significantly.}
\label{tab:pascal_base}
\end{table}


==> assets/tables/pascal_full.tex <==
% !TEX root = ../../main.tex
\begin{table*}[h]
\centering
\begin{adjustbox}{width=0.7\textwidth}
\begin{tabular}{@{}c|c|c|ccc|ccc|ccc@{}}
\toprule
\multirow{2}{*}{Split}   & \multirow{2}{*}{\# shots} & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Overall} & \multicolumn{3}{c|}{Base Class} & \multicolumn{3}{c}{Novel Class} \\
                         &                           &                         & AP       & AP50    & AP75    & AP        & AP50     & AP75     & AP        & AP50     & AP75     \\ \midrule
\multirow{7}{*}{Split 1} & \multirow{4}{*}{3}        & FR~\cite{Kang2019}      & 29.5     & 53.3    & 28.6    & 33.8      & 61.2     & 32.7     & 16.8      & 29.8     & 16.5     \\
                         &                           & TFA w/ fc~\cite{Wang2020}& 41.8     & 67.1    & 45.4    & 48.2      & 76.0     & 53.1     & 22.6      & 40.4     & 22.4     \\
                         &                           & TFA w/ cos~\cite{Wang2020}& 43.7     & 68.5    & 48.3    & 49.8      & 77.3     & 55.4     & 25.4      & 42.1     & 27.0     \\
                         &                           & Ours                    & -        & -       & -       & -         & -        & -        & -         & -        & -        \\ \cmidrule(l){2-12}
                         & \multirow{3}{*}{10}       & TFA w/ fc~\cite{Wang2020}& 42.8     & 69.5    & 46.0    & 47.3      & 75.4     & 51.6     & 29.3      & 52.0     & 29.0     \\
                         &                           & TFA w/ cos~\cite{Wang2020}& 45.8     & 71.3    & 50.4    & 50.4      & 77.5     & 55.9     & 32.0      & 52.8     & 33.7     \\
                         &                           & Ours                    & -        & -       & -       & -         & -        & -        & -         & -        & -        \\ \midrule
\multirow{7}{*}{Split 2} & \multirow{4}{*}{3}        & FR~\cite{Kang2019}      & 29.9     & 53.9    & 29.0    & 35.7      & 63.5     & 35.1     & 12.5      & 25.1     & 10.4     \\
                         &                           & TFA w/ fc~\cite{Wang2020}& 39.4     & 64.2    & 42.0    & 47.5      & 75.4     & 51.7     & 15.2      & 30.5     & 13.1     \\
                         &                           & TFA w/ cos~\cite{Wang2020}& 40.1     & 64.5    & 43.3    & 48.1      & 75.6     & 52.9     & 16.0      & 30.9     & 14.4     \\
                         &                           & Ours                    & -        & -       & -       & -         & -        & -        & -         & -        & -        \\ \cmidrule(l){2-12}
                         & \multirow{3}{*}{10}       & TFA w/ fc~\cite{Wang2020}& 41.3     & 67.0    & 44.0    & 48.3      & 76.1     & 52.7     & 20.2      & 39.7     & 18.0     \\
                         &                           & TFA w/ cos~\cite{Wang2020}& 42.3     & 67.6    & 45.7    & 49.4      & 76.9     & 54.5     & 20.8      & 39.5     & 19.2     \\
                         &                           & Ours                    & -        & -       & -       & -         & -        & -        & -         & -        & -        \\ \midrule
\multirow{7}{*}{Split 3} & \multirow{4}{*}{3}        & FR~\cite{Kang2019}      & 29.2     & 52.7    & 28.5    & 34.2      & 61.3     & 33.6     & 14.2      & 26.8     & 13.1     \\
                         &                           & TFA w/ fc~\cite{Wang2020}& 40.4     & 65.4    & 43.1    & 47.8      & 75.6     & 52.1     & 18.1      & 34.7     & 16.2     \\
                         &                           & TFA w/ cos~\cite{Wang2020}& 43.1     & 67.5    & 46.7    & 51.1      & 78.6     & 56.3     & 18.9      & 34.3     & 18.1     \\
                         &                           & Ours                    & -        & -       & -       & -         & -        & -        & -         & -        & -        \\ \cmidrule(l){2-12}
                         & \multirow{3}{*}{10}       & TFA w/ fc~\cite{Wang2020}& 42.2     & 68.3    & 44.9    & 48.5      & 76.2     & 52.9     & 23.3      & 44.6     & 21.0     \\
                         &                           & TFA w/ cos~\cite{Wang2020}& 45.0     & 70.3    & 48.9    & 51.6      & 78.6     & 57.0     & 25.4      & 45.6     & 24.7     \\
                         &                           & Ours                    & -        & -       & -       & -         & -        & -        & -         & -        & -        \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{3pt}
\caption{Full detection performance in the few-shot setting on the PASCAL VOC dataset. We report three metrics used in MS-COCO for overall, base and novel performance using the 3 different class splits.}
\label{tab:pascal_full}
\end{table*}


==> assets/tables/pascal_new.tex <==
% !TEX root = ../../main.tex
\begin{table*}[htb!]
\centering
\scriptsize
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}l|c|ccccc|ccccc|ccccc@{}}
\toprule
\multirow{2}{*}{Method/Shot}     & \multirow{2}{*}{Backbone}  & \multicolumn{5}{c|}{Novel Split 1} & \multicolumn{5}{c|}{Novel Split 2} & \multicolumn{5}{c}{Novel Split 3} \\
                                 &                            & 1            & 2            & 3            & 5            & 10            & 1             & 2             & 3             & 5             & 10             & 1                & 2              & 3              & 5              & 10             \\ \midrule
YOLOv2-ft~\cite{Kang2019}      \hfill \textit{ICCV 19}     & \multirow{3}{*}{YOLO V2}   & 6.6          & 10.7         & 12.5         & 24.8         & 38.6          & 12.5          & 4.2           & 11.6          & 16.1          & 33.9           & 13.0             & 15.9           & 15.0           & 32.2           & 38.4           \\
FSRW~\cite{Kang2019}           \hfill \textit{ICCV 19}     &                            & 14.8         & 15.5         & 26.7         & 33.9         & 47.2          & 15.7          & 15.3          & 22.7          & 30.1          & 40.5           & 21.3             & 25.6           & 28.4           & 42.8           & 45.9           \\
MetaDet~\cite{Wang2019}        \hfill \textit{ICCV 19}     &                            & 17.1         & 19.1         & 28.9         & 35.0         & 48.8          & 18.2          & 20.6          & 25.9          & 30.6          & 41.5           & 20.1             & 22.3           & 27.9           & 41.9           & 42.9           \\ \midrule
FRCN-ft~\cite{Kang2019}        \hfill \textit{ICCV 19}     & \multirow{4}{*}{FRCN-R101} & 13.8         & 19.6         & 32.8         & 41.5         & 45.6          & 7.9           & 15.3          & 26.2          & 31.6          & 39.1           & 9.8              & 11.3           & 19.1           & 35.0           & 45.1           \\
FRCN+FPN-ft~\cite{Wang2020}    \hfill \textit{ICML 20}     &                            & 8.2          & 20.3         & 29.0         & 40.1         & 45.5          & 13.4          & 20.6          & 28.6          & 32.4          & 38.8           & 19.6             & 20.8           & 28.7           & 42.2           & 42.1           \\
MetaDet~\cite{Wang2019}        \hfill \textit{ICCV 19}     &                            & 18.9         & 20.6         & 30.2         & 36.8         & 49.6          & 21.8          & 23.1          & 27.8          & 31.7          & 43.0           & 20.6             & 23.9           & 29.4           & 43.9           & 44.1           \\
Meta R-CNN~\cite{Yan2019}      \hfill \textit{ICCV 19}     &                            & 19.9         & 25.5         & 35.0         & 45.7         & 51.5          & 10.4          & 19.4          & 29.6          & 34.8          & 45.4           & 14.3             & 18.2           & 27.5           & 41.2           & 48.1           \\ \midrule
TFA w/ fc~\cite{Wang2020}      \hfill \textit{ICML 20}     & \multirow{5}{*}{FRCN-R101} & 36.8         & 29.1         & 43.6         & 55.7         & 57.0          & 18.2          & 29.0          & 33.4          & 35.5          & 39.0           & 27.7             & 33.6           & 42.5           & 48.7           & 50.2           \\
TFA w/ cos~\cite{Wang2020}     \hfill \textit{ICML 20}     &                            & 39.8         & 36.1         & 44.7         & 55.7         & 56.0          & 23.5          & 26.9          & 34.1          & 35.1          & 39.1           & 30.8             & 34.8           & 42.8           & 49.5           & 49.8           \\
MPSR~\cite{Wu2020a}            \hfill \textit{ECCV 20}     &                            & 41.7         & -            & \sbest{51.4} & 55.2         & \sbest{61.8}  & 24.4          & -             & 39.2          & 39.9          & 47.8           & 35.6             & -              & 42.3           & 48.0           & 49.7           \\
FSCE~\cite{Sun2021}            \hfill \textit{CVPR 21}     &                            & \sbest{44.2} & 43.8         & \sbest{51.4} & \best{61.9}  & \best{63.4}   & \sbest{27.3}  & \sbest{29.5}  & \best{43.5}   & \sbest{44.2}  & \best{50.2}    & \sbest{37.2}     & \sbest{41.9}   & \best{47.5}    & \sbest{54.6}   & \best{58.5}    \\
Retentive R-CNN~\cite{Fan2021} \hfill \textit{CVPR 21}     &                            & 42.4         & \sbest{45.8} & 45.9         & 53.7         & 56.1          & 21.7          & 27.8          & 35.2          & 37.0          & 40.3           & 30.2             & 37.6           & 43.0           & 49.7           & 50.1           \\ \midrule
Ours (Baseline)                \hfill                      & \multirow{2}{*}{FRCN-R50}  & 37.7         & 42.0         & 50.3         & 57.0         & 58.0          & 19.8          & 22.5          & 35.6          & 42.7          & 44.1           & 33.9             & 36.0           & 38.6           & 49.8           & 51.6           \\
Ours (After Query Expansion)   \hfill                     &                            & \best{48.9}  & \best{48.4}  & \best{54.2}  & \sbest{60.3} & 61.6          & \best{36.9}   & \best{33.1}   & \sbest{43.4}  & \best{44.4}   & \sbest{48.8}   & \best{42.4}      & \best{46.0}    & \sbest{44.9}   & \best{54.7}    & \sbest{57.4}   \\ \bottomrule
% Ours (Query Expand 2x)     &                      &                            & 47.2  & 44.5  & 51.2 & 56.7 & 58.7 & 33.4  & 31.0  & 36.4 & 42.4 & 44.8 & 40.3  & 34.2 & 41.6 & 50.6 & 53.1 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Few-shot detection performance across the three splits on the PASCAL VOC benchmark. Best and second-best results are coloured \best{blue} and \sbest{red},
respectively.}
\label{tab:pascal_new}
\vspace{-10pt}
\end{table*}


==> assets/tables/pascal_new_post.tex <==
% !TEX root = ../../main.tex
\begin{table*}[htb!]
\centering
\scriptsize
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}l|c|ccccc|ccccc|ccccc@{}}
\toprule
\multirow{2}{*}{Method/Shot}                               & \multirow{2}{*}{Backbone}  & \multicolumn{5}{c|}{Novel Split 1}                                        & \multicolumn{5}{c|}{Novel Split 2}                                             & \multicolumn{5}{c}{Novel Split 3} \\
&         & 1            & 2            & 3            & 5            & 10            & 1             & 2             & 3             & 5             & 10             & 1                & 2              & 3              & 5              & 10             \\ \midrule
YOLOv2-ft~\cite{Kang2019}      \hfill \textit{ICCV 19}     & \multirow{3}{*}{YOLO V2}   & 6.6          & 10.7         & 12.5         & 24.8         & 38.6          & 12.5          & 4.2           & 11.6          & 16.1          & 33.9           & 13.0             & 15.9           & 15.0           & 32.2           & 38.4           \\
FSRW~\cite{Kang2019}           \hfill \textit{ICCV 19}     &                            & 14.8         & 15.5         & 26.7         & 33.9         & 47.2          & 15.7          & 15.3          & 22.7          & 30.1          & 40.5           & 21.3             & 25.6           & 28.4           & 42.8           & 45.9           \\
MetaDet~\cite{Wang2019}        \hfill \textit{ICCV 19}     &                            & 17.1         & 19.1         & 28.9         & 35.0         & 48.8          & 18.2          & 20.6          & 25.9          & 30.6          & 41.5           & 20.1             & 22.3           & 27.9           & 41.9           & 42.9           \\ \midrule
FRCN-ft~\cite{Kang2019}        \hfill \textit{ICCV 19}     & \multirow{4}{*}{FRCN-R101} & 13.8         & 19.6         & 32.8         & 41.5         & 45.6          & 7.9           & 15.3          & 26.2          & 31.6          & 39.1           & 9.8              & 11.3           & 19.1           & 35.0           & 45.1           \\
FRCN+FPN-ft~\cite{Wang2020}    \hfill \textit{ICML 20}     &                            & 8.2          & 20.3         & 29.0         & 40.1         & 45.5          & 13.4          & 20.6          & 28.6          & 32.4          & 38.8           & 19.6             & 20.8           & 28.7           & 42.2           & 42.1           \\
MetaDet~\cite{Wang2019}        \hfill \textit{ICCV 19}     &                            & 18.9         & 20.6         & 30.2         & 36.8         & 49.6          & 21.8          & 23.1          & 27.8          & 31.7          & 43.0           & 20.6             & 23.9           & 29.4           & 43.9           & 44.1           \\
Meta R-CNN~\cite{Yan2019}      \hfill \textit{ICCV 19}     &                            & 19.9         & 25.5         & 35.0         & 45.7         & 51.5          & 10.4          & 19.4          & 29.6          & 34.8          & 45.4           & 14.3             & 18.2           & 27.5           & 41.2           & 48.1           \\ \midrule
TFA w/ fc~\cite{Wang2020}      \hfill \textit{ICML 20}     & \multirow{5}{*}{FRCN-R101} & 36.8         & 29.1         & 43.6         & 55.7         & 57.0          & 18.2          & 29.0          & 33.4          & 35.5          & 39.0           & 27.7             & 33.6           & 42.5           & 48.7           & 50.2           \\
TFA w/ cos~\cite{Wang2020}     \hfill \textit{ICML 20}     &                            & 39.8         & 36.1         & 44.7         & 55.7         & 56.0          & 23.5          & 26.9          & 34.1          & 35.1          & 39.1           & 30.8             & 34.8           & 42.8           & 49.5           & 49.8           \\
MPSR~\cite{Wu2020a}            \hfill \textit{ECCV 20}     &                            & 41.7         & -            &       {51.4} & 55.2         & \sbest{61.8}  & 24.4          & -             & \sbest{39.2}  & 39.9          & \sbest{47.8}   & 35.6             & -              & 42.3           & 48.0           & 49.7           \\
FSCE~\cite{Sun2021}            \hfill \textit{CVPR 21}     &                            &       {44.2} & 43.8         &       {51.4} & \best{61.9}  & \best{63.4}   &  \sbest{27.3} &  \sbest{29.5} & \best{43.5}   &  \best{44.2}  &  \best{50.2}   & \sbest{37.2}     & \sbest{41.9}   &
\best{47.5}    & \best{54.6}    &  \best{58.5}   \\
Retentive R-CNN~\cite{Fan2021} \hfill \textit{CVPR 21}     &                            & 42.4         &       {45.8} & 45.9         & 53.7         & 56.1          & 21.7          & 27.8          & 35.2          & 37.0          & 40.3           & 30.2             & 37.6           & 43.0           & 49.7           & 50.1           \\ \midrule
Ours (Baseline)                \hfill                      & \multirow{3}{*}{FRCN-R50}  & 37.7         & 42.0         & 50.3         & 57.0         & 58.0          & 19.8          & 22.5          & 35.6          & 42.7          & 44.2           & 33.9             & 36.0           & 38.6           & 49.8           & 51.6           \\
%Ours (Query Expansion)   \hfill                            &                            & \best{48.9}  & \sbest{48.4} &      {54.2}  & \sbest{60.3} & 61.6          &  \best{36.9}  & \sbest{33.1}  &  \sbest{43.4} &  \best{44.4}  & \sbest{48.8}   & \best{42.4}      &  \best{46.0}   &  \best{44.9}    &  \best{54.7}   &  \sbest{57.4}  \\ \midrule

Ours (Query Expansion$\dagger$) \hfill                     &                            &  \best{48.2} &  \best{51.7} &  \best{57.1} & \sbest{58.6} & 59.2          &   \best{30.5} &  \best{34.6}  &       {37.7}  & \sbest{43.9}  &       {44.5}   & \best{42.4}      & \best{43.9}   &  \sbest{44.7}   &  \sbest{51.5}   &  \sbest{54.3}  \\
Naive Query Expansion$\ddagger$ \hfill                     &                            & \sbest{44.5} & \sbest{47.5} & \sbest{54.8} &       {52.5} & 56.7          &      {26.1}   &      {27.1}   &       {34.4}  &      {40.8}   &       {42.2}   &      {36.3}      &      {38.1}    &       {40.1}  &      {47.5}    &       {53.5}   \\\bottomrule
% Ours (Query Expand 2x)     &                      &                            & 47.2  & 44.5  & 51.2 & 56.7 & 58.7 & 33.4  & 31.0  & 36.4 & 42.4 & 44.8 & 40.3  & 34.2 & 41.6 & 50.6 & 53.1 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Few-shot detection performance across the three splits on the PASCAL VOC benchmark. Best and second-best results are coloured \best{blue} and \sbest{red},
respectively.}
\label{tab:pascal_new_post}
\vspace{-10pt}
\end{table*}


==> assets/tables/pascal_novel.tex <==
% !TEX root = ../../main.tex
% \begin{table*}[t]
% \centering
% \begin{adjustbox}{width=\textwidth}
% \begin{tabular}{@{}l|c|ccccc|ccccc|ccccc@{}}
% \toprule
% \multirow{2}{*}{Method / Shots} & \multirow{2}{*}{Backbone} & \multicolumn{5}{c|}{Novel Set 1}                                                                                                                        & \multicolumn{5}{c|}{Novel Set 2}                                                                                                               & \multicolumn{5}{c}{Novel Set 3}                                                                                                      \\
%                                 &                           & 1                                 & 2                                 & 3                        & 5                        & 10                        & 1                        & 2                                 & 3                        & 5                        & 10                        & 1                        & 2                        & 3                        & 5                        & 10                       \\ \midrule
% FR~\cite{Kang2019}              & YOLOv2 w/ DarkNet-19      & 14.8                              & 15.5                              & 26.7                     & 33.9                     & 47.2                      & 15.7                     & 15.3                              & 22.7                     & 30.1                     & 40.5                      & \textbf{21.3}            & 25.6                     & 28.4                     & 42.8                     & 45.9                     \\
% MetaDet~\cite{Wang2019}         & FRCN w/ VGG16             & 18.9                              & 20.6                              & 30.2                     & 36.8                     & 49.6                      & \textbf{21.8}            & 23.1                              & 27.8                     & 31.7                     & 43.0                      & 20.6                     & 23.9                     & 29.4                     & 43.9                     & 44.1                     \\
% Meta R-CNN~\cite{Yan2019}       & FRCN w/ R-101             & 19.9                              & 25.5                              & 35.0                     & 45.7                     & 51.5                      & 10.4                     & 19.4                              & 29.6                     & 34.8                     & 45.4                      & 14.3                     & 18.2                     & 27.5                     & 41.2                     & 48.1                     \\
% TFA w/ fc~\cite{Wang2020}       & FRCN w/ R-101             & 22.9                              & 34.5                              & 40.4                     & 46.7                     & 52.0                      & 16.9                     & 26.4                              & 30.5                     & 34.6                     & 39.7                      & 15.7                     & 27.2                     & 34.7                     & 40.8                     & 44.6                     \\
% TFA w/ cos~\cite{Wang2020}      & FRCN w/ R-101             & \multicolumn{1}{l}{\textbf{25.3}} & \multicolumn{1}{l}{\textbf{36.4}} & \multicolumn{1}{l}{42.1} & \multicolumn{1}{l}{47.9} & \multicolumn{1}{l|}{52.8} & \multicolumn{1}{l}{18.3} & \multicolumn{1}{l}{\textbf{27.5}} & \multicolumn{1}{l}{30.9} & \multicolumn{1}{l}{34.1} & \multicolumn{1}{l|}{39.5} & \multicolumn{1}{l}{17.9} & \multicolumn{1}{l}{27.2} & \multicolumn{1}{l}{34.3} & \multicolumn{1}{l}{40.8} & \multicolumn{1}{l}{45.6} \\
% FSOD-VE~\cite{Xiao2020}         & FRCN w/ R-101             & 24.2                              & 35.3                              & \textbf{42.2}            & \textbf{49.1}            & \textbf{57.4}             & 21.6                     & 24.6                              & \textbf{31.9}            & \textbf{37.0}            & \textbf{45.7}             & 21.2                     & \textbf{30.0}            & \textbf{37.2}            & \textbf{43.8}            & \textbf{49.6}            \\
% Ours                            & FCOS w/ R-50              & -                                 & -                                 & -                        & -                        & -                         & -                        & -                                 & -                        & -                        & -                         & -                        & -                        & -                        & -                        & -                        \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \vspace{3pt}
% \caption{Few-shot detection performance (mAP50) on the PASCAL VOC dataset. FRCN denotes Faster R-CNN. We report results under 3 different splits for 5 novel classes.}
% \label{tab:pascal_novel}
% \end{table*}

\begin{table*}[h]
\centering
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}l|c|ccccc|ccccc|ccccc@{}}
\toprule
\multirow{2}{*}{Method / Shots} & \multirow{2}{*}{Backbone}             & \multicolumn{5}{c|}{Novel Set 1}                                              & \multicolumn{5}{c|}{Novel Set 2}                                              & \multicolumn{5}{c}{Novel Set 3}                                               \\
                                &                                       & 1             & 2             & 3             & 5             & 10            & 1             & 2             & 3             & 5             & 10            & 1             & 2             & 3             & 5             & 10            \\ \midrule
YOLO-joint*~\cite{Kang2019}     & \multirow{5}{*}{YOLOv2 w/ DarkNet-19} & 0.0           & 0.0           & 1.8           & 1.8           & 1.8           & 0.0           & 0.1           & 0.0           & 1.8           & 0.0           & 1.8           & 1.8           & 1.8           & 3.6           & 3.9           \\
YOLO-ft*~\cite{Kang2019}        &                                       & 3.2           & 6.5           & 6.4           & 7.5           & 12.3          & 8.2           & 3.8           & 3.5           & 3.5           & 7.8           & 8.1           & 7.4           & 7.6           & 9.5           & 10.5          \\
YOLO-ft-full*~\cite{Kang2019}   &                                       & 6.6           & 10.7          & 12.5          & 24.8          & 38.6          & 12.5          & 4.2           & 11.6          & 16.1          & 33.9          & 13.0          & 15.9          & 15.0          & 32.2          & 38.4          \\
FR*~\cite{Kang2019}             &                                       & 14.8          & 15.5          & 26.7          & 33.9          & 47.2          & 15.7          & 15.3          & 22.7          & 30.1          & 40.5          & \textbf{21.3} & 25.6          & 28.4          & 42.8          & 45.9          \\
MetaDet~\cite{Wang2019}         &                                       & 17.1          & 19.1          & 28.9          & 35.0          & 48.8          & 18.2          & 20.6          & 25.9          & 30.6          & 41.5          & 20.1          & 22.3          & 27.9          & 41.9          & 42.9          \\ \midrule
FRCN-joint~\cite{Wang2019}      & \multirow{3}{*}{FRCN w/ VGG16}        & 0.3           & 0.0           & 1.2           & 0.9           & 1.7           & 0.0           & 0.0           & 1.1           & 1.9           & 1.7           & 0.2           & 0.5           & 1.2           & 1.9           & 2.8           \\
FRCN-ft~\cite{Wang2019}         &                                       & 9.1           & 10.9          & 13.7          & 25.0          & 39.5          & 10.9          & 13.2          & 17.6          & 19.5          & 36.5          & 15.0          & 15.1          & 18.3          & 33.1          & 35.9          \\
MetaDet~\cite{Wang2019}         &                                       & 18.9          & 20.6          & 30.2          & 36.8          & 49.6          & \textbf{21.8} & 23.1          & 27.8          & 31.7          & 43.0          & 20.6          & 23.9          & 29.4          & 43.9          & 44.1          \\ \midrule
FRCN-joint~\cite{Yan2019}       & \multirow{4}{*}{FRCN w/ R-101}        & 2.7           & 3.1           & 4.3           & 11.8          & 29.0          & 1.9           & 2.6           & 8.1           & 9.9           & 12.6          & 5.2           & 7.5           & 6.4           & 6.4           & 6.4           \\
FRCN-ft~\cite{Yan2019}          &                                       & 11.9          & 16.4          & 29.0          & 36.9          & 36.9          & 5.9           & 8.5           & 23.4          & 29.1          & 28.8          & 5.0           & 9.6           & 18.1          & 30.8          & 43.4          \\
FRCN-ft-full~\cite{Yan2019}     &                                       & 13.8          & 19.6          & 32.8          & 41.5          & 45.6          & 7.9           & 15.3          & 26.2          & 31.6          & 39.1          & 9.8           & 11.3          & 19.1          & 35.0          & 45.1          \\
Meta R-CNN~\cite{Yan2019}       &                                       & 19.9          & 25.5          & 35.0          & 45.7          & 51.5          & 10.4          & 19.4          & 29.6          & 34.8          & 45.4          & 14.3          & 18.2          & 27.5          & 41.2          & 48.1          \\ \midrule
FRCN-ft-full~\cite{Wang2020}    & \multirow{3}{*}{FRCN w/ R-101}        & 15.2          & 20.3          & 29.0          & 40.1          & 45.5          & 13.4          & 20.6          & 28.6          & 32.4          & 38.8          & 19.6          & 20.8          & 28.7          & 42.2          & 42.1          \\
TFA w/ fc~\cite{Wang2020}       &                                       & 22.9          & 34.5          & 40.4          & 46.7          & 52.0          & 16.9          & 26.4          & 30.5          & 34.6          & 39.7          & 15.7          & 27.2          & 34.7          & 40.8          & 44.6          \\
TFA w/ cos~\cite{Wang2020}      &                                       & \textbf{25.3} & \textbf{36.4} & 42.1          & 47.9          & 52.8          & 18.3          & \textbf{27.5} & 30.9          & 34.1          & 39.5          & 17.9          & 27.2          & 34.3          & 40.8          & 45.6          \\ \midrule
FSOD-VE~\cite{Xiao2020}         & FRCN w/ R-101                         & 24.2          & 35.3          & \textbf{42.2} & \textbf{49.1} & \textbf{57.4} & 21.6          & 24.6          & \textbf{31.9} & \textbf{37.0} & \textbf{45.7} & 21.2          & \textbf{30.0} & \textbf{37.2} & \textbf{43.8} & \textbf{49.6} \\ \midrule
Ours                            & FPN w/ R-50                          & -             & -             & -             & -             & -             & -             & -             & -             & -             & -             & -             & -             & -             & -             & -             \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{3pt}
\caption{Few-shot detection performance (mAP50) on the PASCAL VOC dataset. FRCN denotes Faster R-CNN. We report results under 3 different splits for 5 novel classes. *Results are \emph{not} averaged over multiple runs.}
\label{tab:pascal_novel}
\end{table*}


==> assets/tables/query_expansion_steps.tex <==
% !TEX root = ../../main.tex
\begin{table}[!htb]
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}l|ccc|ccc@{}}
\toprule
Method               & nAP  & nAP50 & nAP75 & bAP  & bAP50 & bAP75 \\ \midrule
Baseline             & 16.6 & 30.9  & 15.8  & 29.5 & 46.7  & 32.4  \\
+ Pseudo-Labelling   & 18.4 & 34.0  & 18.2  & 31.7 & 53.2  & 35.6  \\
+ Label Verification & 21.8 & 40.3  & 21.1  & 31.6 & 53.4  & 35.2  \\
+ Box Correction     & 25.5 & 42.0  & 27.3  & 33.3 & 53.6  & 36.1  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-5pt}
\captionof{table}{Demonstration of the benefit of each step of pseudo-labelling method.}
\label{tab:ablation_qe_steps}
\end{table}


==> assets/tables/tfa-rpn-ft.tex <==



% ==================================================
\begin{table*}[t]
\scriptsize
\begin{minipage}[t]{.48\linewidth}
\centering
\setlength\tabcolsep{6pt}
\begin{tabular}[t]{@{}lc|c|ccc@{}}
\toprule
Method                            & Backbone & Data    & nAP                         & nAP50                       & nAP75                       \\ \midrule
TFA~\cite{Wang2020}        & R101     & 10-shot & {\color[HTML]{000000} 10.0} & {\color[HTML]{000000} 19.1} & {\color[HTML]{000000} 9.3}  \\
TFA~\cite{Wang2020}        & R50      & 10-shot & 9.5                         & 18.8                        & 8.9                         \\
TFA~\cite{Wang2020}        & R101     & 30-shot & {\color[HTML]{000000} 13.7} & {\color[HTML]{000000} 24.9} & {\color[HTML]{000000} 13.4} \\
TFA~\cite{Wang2020}        & R50      & 30-shot & 13.0                        & 24.7                        & 12.3                        \\
TFA~\cite{Wang2020}        & R50      & all     & 18.3                        & 33.3                        & 17.7                        \\
Faster R-CNN~\cite{Ren16,Wu2019a} & R50      & all     & 43.5                        & 67.4                        & 46.6                        \\ \bottomrule
\end{tabular}
\caption{
Investigation on the transferability of base features to novel instance detection.
TFA and an equivalent Faster R-CNN model are both trained on MS-COCO,
with different amounts of novel training instances.
The best performance TFA can achieve with access to all data (penultimate row, $18.3$ nAP) is significantly
lower than the capacity of an equivalent model trained fully (final row, $43.5$ nAP).}
\label{tab:tfa_limit}
\end{minipage}
% ==================================================
\hfill
\begin{minipage}[t]{.5\linewidth}
\scriptsize
\setlength\tabcolsep{4pt}
\begin{tabular}[t]{@{}lc|cc@{}}
\toprule
RPN Training                                    & \begin{tabular}[c]{@{}c@{}}No.\\ Proposals\end{tabular} & nAR\textsubscript{IoU=0.5} & $\min$(R50\textsubscript{IoU=0.5}) \\ \midrule
Pretrained on base data only~\cite{Wang2020}    & 100      & 49.7    & 16.2      \\
Finetuned on novel data ($30$ shots only)           & 100     & 71.0     & 40.0      \\
Pretrained on all data~\cite{Ren16,Wu2019a}      & 100      & 84.0     & 64.5      \\ \midrule
Pretrained on base data only~\cite{Wang2020}    & 1000    & 82.1     & 55.9     \\
Finetuned on novel data ($30$ shots only)          & 1000    & 88.5     & 77.0      \\
Pretrained on all data~\cite{Ren16,Wu2019a}     & 1000     & 95.0     & 79.2     \\ \bottomrule
\end{tabular}
\caption{
RPN recall of novel instances on COCO, using an IoU=$0.5$ criterion.
nAR50 -- novel class average recall, min(nR50) -- minimum novel class recall. RPN finetuning is performed using 30-shots.
Training an RPN on base class data only leads to poor recall on novel classes.}
\label{tab:rpn_finetune}
\end{minipage}
\end{table*}
% ==================================================




==> sections/06-limit.tex <==
% !TEX root = ../main.tex
\section{Limitations}
\label{sec:limitation}

** I suggest we just have this in the supplementary. Instead of this section, we  could have a statement such as

``We discuss potential ethical concerns and limitations of our work in the Supplementary Material.
Upon publication we will make the code and pre-trained models of this work public.''

at the end of the intro
**

There are two main limitations of our work:
{\em first}, our work only performs one iteration of pseudo-labelling
and end-to-end re-training and we find that performing extra iterations of our method
does not improve benchmark performance;
{\em second}, we make use of `{\em ignore regions}' for the cases where some novel instances in
an image do not have a pseudo-annotations -- ideally we would not make use of these ignore regions.
The Supplementary Material contains a discussion of these limitations.


==> sections/fw.tex <==
% !TEX root = ../main.tex
\section{Future Work}
Prior to conference submission,
there are more methods to be explored;
these are presented in Section~\ref{ssec:future_methods}.
Moreover, we need to benchmark our model on other existing datasets,
\eg~Pascal-VOC, and LVIS~\cite{Gupta2019},
which naturally contains many \emph{rare} classes, making it a perfect dataset for benchmarking few-shot object detection approaches.

\subsection{Future Methods}
\label{ssec:future_methods}
To improve the current method presented in Section~\ref{sec:method},
we have a number of improvements which are to be investigated in future.
These are: (i) including self-supervised training episodes to improve generalisation and prevent novel classes being suppressed into background;
(ii) utilising query expansion techniques from image retrieval to search for unlabelled instances in the dataset,
and bring them into the training process;
(iii) improving the exemplar embedding by making use of attention-based models, \eg~Transformers~\cite{Vaswani17},
such that more informative regions of given exemplars are highlighted,
and the process of synthesising classifiers can be conditioned on the target image.

\subsubsection{Self-supervised Training for Generalization}
\label{sssec:self_sup}
Comparing with standard object detection problems,
we conjecture the
challenge for few-shot object detection arises from the drastic imbalance in available data between base and \new categories,
\ie~object instances belonging to \new categories may be present in the image without being annotated,
therefore being treated as background during training.
As a result, CNNs trained through classical supervised learning tend to over-specialize on the base categories
and treat these \new categories as genuine background, suppressing the discriminative information in these regions.

To overcome this problem,
we propose a conceptually simple self-supervised learning method as part of base training.
Given a target image $I_t$,
we take an augmentation (or multiple different augmentations) of a crop in the image,
and use this as input to the exemplar stream.
The target image $I_t$ is used as input to the image stream.
In self-supervised iterations, the goal is for the model to match the instance,
shown in the crop(s), back to the source image using Equation~\ref{eq:sim}.

We hypothesise that if the model is successful at the instance matching task,
the image stream must retain as much information as possible about natural images,
instead of over-specialising on the base categories, thereby circumventing \new instance suppression.
In practice, to improve the likelihood of salient objects occurring in crops,
we propose to use the unsupervised selective search region proposal method~\cite{Uijlings2013} to get the crops that potentially contain objects.
%Furthermore, as we treat bounding box regression as class-agnostic,
%this is not attended to in instance matching iterations; we would only compute the first term of Equation~\ref{eq:loss}.

\subsubsection{Query Expansion}
\label{sssec:query_exp}
In object detection, multiple objects exist in a single image.
In few-shot object detection, for \new categories there are only limited annotations available.
However, it is plausible that unlabelled instances of \new categories are also present in the the base training data images $D_{\text{b}}$.
We propose to use query expansion techniques, widely used in image retrieval~\cite{Chum07b,Chum11}.
By leveraging the limited \new annotations available $B_{\text{n}}$,
we aim to expand the number of annotations available for \new classes by searching base training images $D_{\text{b}}$, for such objects.
With expanded annotations, we can therefore take the benefits of increased labelled data in supervised settings.

Similarly, this query expansion can also be applied at inference time.
Specifically, after finetuning on base and novel categories $C_{\text{b}} \cup C_{\text{n}}$ using a balanced dataset,
we possess a mean feature vector $\tilde{\mathbf{t}}_c$ for each novel category.
These features can be used to infer bounding box proposals for \new objects.
The highest scoring bounding box proposals can be included as new annotations from which further finetuning can take place.
Given large image datasets, this process can be repeated multiple times to include new annotations as training data.

\subsubsection{Exemplar Aggregation}
\label{sssec:set_rep}
At inference time,
our current method uses a simple average of the given exemplar embeddings $\tilde{\mathbf{t}}$ as a classification vector for each class.
To generate more informative feature aggregation with the given exemplars,
we also plan to make use of attention-based modules~\cite{Vaswani17}.
We propose to use feature maps with spatial resolution as exemplar embeddings,
rather than a single vector.
This will allow for spatial attention within and between exemplars,
as well as on the target image,
highlighting the most informative regions of the object exemplars, conditioned on the target image.

\subsection{Future Benchmarks and Datasets}
Last but not least, there are existing benchmarks for which we do not have results yet.
These benchmarks are on Pascal VOC and LVIS.
For Pascal VOC, we propose to follow the experimental setup in~\cite{Kang2019},
using the same three base and novel class splits of the $20$ classes available in Pascal VOC.
The number of shots available for each novel class are $K=1,2,3,5,10$.
For LVIS, we propose to follow the experimental setup in~\cite{Wang2020},
in which the frequent and common classes in the vocabulary of LVIS are used as base classes
and rare classes are used as novel classes, with $K=10$ shots available for each rare class.

%\subsection{Ablation Study}
%\label{ssec:ablation}
% \input{assets/tables/pascal_novel.tex}
% \input{assets/tables/pascal_full.tex}
% \input{assets/tables/pascal_base.tex}
% \input{assets/tables/coco_novel.tex}
% \input{assets/tables/coco_full.tex}
% \input{assets/tables/lvis_full.tex}

%\paragraph{Self-supervised Training}

%\paragraph{Query Expansion}


==> sections/results.tex <==
% !TEX root = ../main.tex

\section{Results}
\label{sec:results}

In this section,
we demonstrate our approach on MS-COCO~\cite{Lin14}, comparing with previous works, and discuss the current results.

\subsection{Two-stream Few-shot Object Detection}
\label{ssec:exist_fsod}

\paragraph{Baselines}
We compare our approach with existing models attending to few-shot object detection:
\texttt{FR}~\cite{Kang2019},
\texttt{MetaDet}~\cite{Wang2019},
\texttt{Meta R-CNN}~\cite{Yan2019},
\texttt{TFA w/ fc}~\cite{Wang2020},
\texttt{TFA w/ cos}~\cite{Wang2020}
and \texttt{FSOD-VE}~\cite{Xiao2020}.
Furthermore, we compare to a baseline which finetunes a standard object detection model, denoted as \texttt{FRCN+ft-full} where a Faster R-CNN model is trained on base classes and the whole model is subsequently finetuned on novel classes.

\input{assets/tables/coco_novel_bmvc.tex}

\input{assets/tables/pascal_new.tex}
\paragraph{Quantitative Results on MS-COCO}
In both the $10$ and $30$ shot scenarios,
our initial results, shown in Table~\ref{tab:coco_novel}, achieve $4.9$ and $8.2$ respectively,
in terms of novel AP, demonstrating around a $4$ point performance gap,
to the current state-of-the-art method that reports full results~\cite{Wang2020}.
However, it should be noted that our model makes use of a smaller ResNet-50 backbone,
compared to state-of-the-art works which use ResNet-101 architectures.
Another phenomena to notice is,
our approach does not show significant performance degradation on base class performance after finetuning on novel classes,
as shown by the comparison on base classes between stage-1 training and full finetuning,
\eg~30.4 vs.~28.6 with 10 shots,
where stage-1 training refers to the model only trained by base categories,
and full finetuning denotes the model being further finetuned with novel categories.


\paragraph{Query expansion on COCO.}
\weidi{blabla}
\begin{figure}[b]
\includegraphics[width=.45\textwidth]{assets/images/qe.png}
\caption{Placeholder for the query expansion curve, showing 1st, 2nd, 3rd}
\end{figure}


\paragraph{Qualitative Results on COCO.}

\weidi{discuss it.}

\begin{figure*}[t]
\includegraphics[width=\textwidth]{assets/images/teaser.png}
\caption{Placeholder for qualitative results, before query expansion, after query expansion,
may be also failure case, depending on space.}
\end{figure*}

\paragraph{Quantitative Results on Pascal VOC}

\weidi{
blabla
}













\begin{comment}
\subsection{Self-supervised Models in Exemplar Stream}
\label{ssec:evaluating_selfsup}

To prevent our model from over-fitting to base categories and maintain generalisability to \new classes,
we make use of self-supervised pretrained models for the exemplar stream.
Self-supervised models have been shown to be robust to supervision collapse~\cite{Doersch2020},
where predictions of supervised models are heavily biased towards the (dominant) training classes.

To verify the suitability of self-supervised models, we follow three steps: (i) a self-supervised model is trained on ImageNet~\cite{Deng09} using a given self-supervision method (we do not implement this step and instead use the publicly available pretrained models which have demonstrated strong performance); (ii) a classifier is learnt on top of the self-supervised features, trained to classify exemplars sourced from MS-COCO~\cite{Lin14}; (iii) performance is measured by classifying a held out set of exemplars also sourced from MS-COCO.



We formulate two versions of this experiment.
First, we train a model using abundant exemplars sourced from MS-COCO.
Second, we train a model using $K$ exemplars randomly sampled from MS-COCO.
In all cases we withhold $50$ exemplars for each class to use as a test set for inference.

In the first version we vary the complexity of the classifier, either a linear classifier or 2-layer multilayer perception (MLP), and also whether the last residual block (LRB) of the self-supervised model is kept frozen or not.
Furthermore, we compare two popular, high performing self-supervised models.
In the second set of experiments we take the best performing model from the previous experiment and vary the number of exemplars $K$ available for training. We also toggle the classifier form and training of the LRB as in the first experiment, observing the effect of $K$ on the various model forms.
% ** need to clearly define the task first, i.e.\ train on X using self-supervision (where X specifies dataset), then
% test by classification on Y (Y here is COCO). After specifying task, state what will be compared/varied **

% To verify the suitability of such self-supervised models,
% we train conventional classifiers on top of a given self-supervised model with varying layer parameters kept fixed.
% We perform these classification experiments on two different datasets sourced from MS-COCO.
% First, we train a conventional classifier with exemplars sourced from the abundant data available for base categories.
% In the second set of experiments, we sample $K$ shots from all categories and train classifiers.


\subsubsection{Exemplar Construction}
\label{sssec:template_construction}
During training, to construct an object template, we crop a source image using a given bounding box.
The corners of this box are shifted by $[-0.1,0.2]$ relative to the box size.
Furthermore, colour jitter, random grayscaling and horizontal flipping are used for further augmentation.
The resulting crop is padded, using the mean RGB value,
to give a square image which is resized to $224\times224$ to match the input conditions of the original self-supervised model.
At inference, we do not use colour jitter, grayscaling or flipping and use a constant corner shift of $0.1$.
These settings are held constant for all subsequent experiments.

\subsubsection{Exemplar Stream Implementation}
\label{sssec:template_implementation}
Following many self-supervised works~\cite{Noroozi16,Gidaris18,He2020} we use a ResNet-50 architecture~\cite{He16}.
We train three variants of this architecture (all other parameters are frozen):
(i) linear classifier after global average pooling,
(ii) 2-layer multilayer perceptron after global average pooling,
(iii) 2-layer multilayer perceptron with the last residual block finetuned.

\input{assets/tables/template_oracle_large.tex}
\input{assets/tables/template_oracle_shots.tex}

\subsubsection{Exemplar Stream Results}
\label{sssec:template_results}
Table~\ref{tab:template_oracle_large} compares the performance, in our large scale setting,
between two recent self-supervised learning models which demonstrate strong performance on the ImageNet classification~\cite{Deng09} benchmark commonly used in self-supervised learning.
We note that the MoCov2~\cite{Chen2020b} improves substantially as more layers are trained,
indicating the relatively low transferability of the frozen self-supervised features to new datasets (\ie MS-COCO in this case) when compared to the second model tested SwAV~\cite{Caron2020}.
This model outperforms the MoCo model regardless of which layers are trained and critically the increase in performance is small as more layers are trained.

Table~\ref{tab:template_oracle_shots} demonstrates the performance of the best performing model from the previous experiment, namely SwAV, in the few-shot regime.
The generalisability of these self-supervised features are further illustrated by a simple linear classifier producing the best performance, for all values of $K$.
This demonstrates the benefit of self-supervision over strong-supervision in the few-shot regime.
% Confusingly, we do not observe a monotonic decrease in performance as more layers are trained.

% ** isn't the purpose of this to demonstrate the benefit of self-supervision over strong-supervision? If so, this should be the main result here **

\subsubsection{Conclusions for Few-shot Object Detection} % (fold)
\label{sssec:template_conclusions}
The results presented in this section demonstrate that self-supervised features are effective at producing template feature vectors in Fig.~\ref{fig:network} either in the case of plentiful training data or in the few-shot case.
Although our detection model utilizes matching and these experiments illustrate the effectiveness of self-supervised feature in classification,
human face recognition demonstrates the ability of features learnt for face identification (classification) can generalise successfully to face verification (matching)~\cite{Deng2019,Wang2018a}.

% \prannay{Although our detection model uses matching and these experiments illustrate its effectiveness in classification, a recent work in few-shot image classification demonstrates that embeddings learnt by classification can generalise to  scenarios~\cite{Tian2020}. Need to properly form this argument, perhaps something about an upper bound}.
Given a linear layer on top of the SwAV model produces the best performance in the few-shot case (Table~\ref{tab:template_oracle_shots})
and comparable performance to `MLP+LRB' in the large scale case (Table~\ref{tab:template_oracle_large}),
for the exemplar stream we use a ResNet-50 architecture with weights from the SwAV pretrained model and add a simple linear projection after the global average pooling step.
This linear projection is the only trainable parameter in the exemplar stream.
\end{comment}





% Furthermore, we compare to baselines which finetune of standard object detection models: \emph{joint training},
% marked as \texttt{FRCN/YOLO-joint}~\cite{Kang2019,Yan2019,Wang2020,Wang2019},
% which train on base and novel classes in one stage,
% and \emph{finetuning methods}, denoted as \texttt{YOLO/FRCN+ft-full} or \texttt{YOLO/FRCN+ft} depending on number of finetuning iterations,
% where the whole model is finetuned in the second stage of training. \texttt{FRCN} indicates Faster R-CNN~\cite{Ren16}.

% \paragraph{Results on Pascal VOC}
% We provide the performance in terms of average AP50 across novel classes, for three random class splits, in Table~\ref{tab:pascal_novel}.
% Our approach uses a smaller ResNet-50 backbone compared to the best performing previous works~\texttt{TFA} and ~\texttt{FSOD-VE} which use ResNet-101.
% This represents a $45$\% reduction in the number of backbone parameters.
% Furthermore, we make use of an adapted FCOS one-stage architecture, whereas most previous works use a two-stage Faster R-CNN architecture, yielding improved performance in terms of FPS.

% Despite our simpler architecture and smaller network, \textcolor{red}{our approach (last row of Table~\ref{tab:pascal_novel}) outperforms all previous works across all class splits and number of training shots.}
% To illustrate the retention of base class knowledge when finetuning on novel data we also give results for \texttt{base only} in Table~\ref{tab:pascal_base}.
% When compared to \texttt{base only}, which is expected to have the best base class performance as it is trained solely for these classes,
% our full model only has a \textcolor{red}{abc} point performance degradation on base classes,
% illustrating the ability of our model to retain high performance on abundant training data and generalise to novel classes.

% For a more comprehensive comparison, we report our performance across more metrics, and that of available prior works, on base and novel classes in Table~\ref{tab:pascal_full}.
% \textcolor{red}{These results demonstrate that our model has higher performance on base and novel classes across all metrics than previous available works.}


==> sections/sm_sections/00-sm-metadata.tex <==
% !TEX root = ../supplementary_material.tex
\title{\textsc{Label, Verify, Correct: \\A Simple Few Shot Object Detection Method \\[5pt]
               (Supplementary Material)}}

\author{Prannay Kaul \qquad Weidi Xie \qquad Andrew Zisserman\\
Visual Geometry Group, University of Oxford\\
{\tt\small \{prannay, weidi, az\}@robots.ox.ac.uk}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
}


==> sections/sm_sections/00a-plan.tex <==
% !TEX root = ../supplementary_material.tex
\section{Plan}

\subsection{Mentioned in the Paper}
\subsubsection{Limitations}
\begin{itemize}
    \item Experiments for LVIS which is a larger vocabulary expansion
    \item Ignore regions - can we somehow enforce images to be fully labelled
    \item Multiple iterations of the method - noisy label learning/clustering instead
\end{itemize}
\subsubsection{Ethical Concerns}

\subsubsection{Supervision Collapse}
\paragraph{False Positives - Class confusion}
\paragraph{False Negatives - Poor recall}
\begin{itemize}
    \item First show the lack of RPN recall with base trained RPN
    \item Missed detections: TFA vs. Our Baseline vs. Ideal Faster R-CNN (same images)
\end{itemize}

\subsubsection{Ignore Regions}
\begin{itemize}
    \item Show images with:
    \begin{itemize}
        \item pseudo-annotations with all examples labelled (no need for ignore regions)
        \item pseudo-annotations with some examples missing (no ignore regions visible)
        \item pseudo-annotations with some exampels missing (ignore regions visible and their utility shown)
    \end{itemize}
    \item Ablation: Table w/ our model with and without ignore regions
\end{itemize}



% \begin{figure*}[!htb]
% \centering
% \scriptsize
% \includegraphics[width=\linewidth]{sm_assets/sm_images/rpn_base_ft.pdf}
% \vspace{-0.4cm}
% \caption{
% \hl{TODO} RPN trained only on Base vs RPN finetuned on novel data}
% % \caption{\hl{TO DO}}
% \label{fig:rpn_base_ft}
% \end{figure*}

% \begin{figure*}[!htb]
% \centering
% \scriptsize
% \includegraphics[width=\linewidth]{sm_assets/sm_images/fast_rcnn_supervision_collapse.pdf}
% \vspace{-0.4cm}
% \caption{
% \hl{TODO} TFA incorrectly puts positive RPN proposals into background, our modifications to training prevent this form of supervision collapse}
% % \caption{\hl{TO DO}}
% \label{fig:tfa_supervision_collapse}
% \end{figure*}

\subsubsection{}

